Uncertainty analysis for accurate ground truth trajectories with robotic total stations

In the context of robotics, accurate ground truth positioning is essential for the development of Simultaneous Localization and Mapping (SLAM) and control algorithms. Robotic Total Stations (RTSs) provide accurate and precise reference positions in different types of outdoor environments, especially when compared to the limited accuracy of Global Navigation Satellite System (GNSS) in cluttered areas. Three RTSs give the possibility to obtain the six-Degrees Of Freedom (DOF) reference pose of a robotic platform. However, the uncertainty of every pose is rarely computed for trajectory evaluation. As evaluation algorithms are getting increasingly precise, it becomes crucial to take into account this uncertainty. We propose a method to compute this six-DOF uncertainty from the fusion of three RTSs based on Monte Carlo (MC) methods. This solution relies on point-to-point minimization to propagate the noise of RTSs on the pose of the robotic platform. Five main noise sources are identified to model this uncertainty: noise inherent to the instrument, tilt noise, atmospheric factors, time synchronization noise, and extrinsic calibration noise. Based on extensive experimental work, we compare the impact of each noise source on the prism uncertainty and the final estimated pose. Tested on more than 50 km of trajectories, our comparison highlighted the importance of the calibration noise and the measurement distance, which should be ideally under 75 m. Moreover, it has been noted that the uncertainty on the pose of the robot is not prominently affected by one particular noise source, compared to the others.

==> media/mc-ptp/grid.tex <==
\makeatletter
\def\grd@save@target#1{%
  \def\grd@target{#1}}
\def\grd@save@start#1{%
  \def\grd@start{#1}}
\tikzset{
  grid with coordinates/.style={
    to path={%
      \pgfextra{%
        \edef\grd@@target{(\tikztotarget)}%
        \tikz@scan@one@point\grd@save@target\grd@@target\relax
        \edef\grd@@start{(\tikztostart)}%
        \tikz@scan@one@point\grd@save@start\grd@@start\relax
        \draw[minor help lines] (\tikztostart) grid (\tikztotarget);
        \draw[major help lines] (\tikztostart) grid (\tikztotarget);
        \grd@start
        \pgfmathsetmacro{\grd@xa}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@ya}{\the\pgf@y/1cm}
        \grd@target
        \pgfmathsetmacro{\grd@xb}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@yb}{\the\pgf@y/1cm}
        \pgfmathsetmacro{\grd@xc}{\grd@xa + \pgfkeysvalueof{/tikz/grid with coordinates/major step}}
        \pgfmathsetmacro{\grd@yc}{\grd@ya + \pgfkeysvalueof{/tikz/grid with coordinates/major step}}
        \foreach \x in {\grd@xa,\grd@xc,...,\grd@xb}
        \node[anchor=north] at (\x,\grd@ya) {\pgfmathprintnumber{\x}};
        \foreach \y in {\grd@ya,\grd@yc,...,\grd@yb}
        \node[anchor=east] at (\grd@xa,\y) {\pgfmathprintnumber{\y}};
      }
    }
  },
  minor help lines/.style={
    help lines,
    step=\pgfkeysvalueof{/tikz/grid with coordinates/minor step}
  },
  major help lines/.style={
    help lines,
    line width=\pgfkeysvalueof{/tikz/grid with coordinates/major line width},
    step=\pgfkeysvalueof{/tikz/grid with coordinates/major step}
  },
  grid with coordinates/.cd,
  minor step/.initial=.2,
  major step/.initial=1,
  major line width/.initial=2pt,
}
\makeatother



==> media/traj-mc-ptp/grid.tex <==
\makeatletter
\def\grd@save@target#1{%
  \def\grd@target{#1}}
\def\grd@save@start#1{%
  \def\grd@start{#1}}
\tikzset{
  grid with coordinates/.style={
    to path={%
      \pgfextra{%
        \edef\grd@@target{(\tikztotarget)}%
        \tikz@scan@one@point\grd@save@target\grd@@target\relax
        \edef\grd@@start{(\tikztostart)}%
        \tikz@scan@one@point\grd@save@start\grd@@start\relax
        \draw[minor help lines] (\tikztostart) grid (\tikztotarget);
        \draw[major help lines] (\tikztostart) grid (\tikztotarget);
        \grd@start
        \pgfmathsetmacro{\grd@xa}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@ya}{\the\pgf@y/1cm}
        \grd@target
        \pgfmathsetmacro{\grd@xb}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@yb}{\the\pgf@y/1cm}
        \pgfmathsetmacro{\grd@xc}{\grd@xa + \pgfkeysvalueof{/tikz/grid with coordinates/major step}}
        \pgfmathsetmacro{\grd@yc}{\grd@ya + \pgfkeysvalueof{/tikz/grid with coordinates/major step}}
        \foreach \x in {\grd@xa,\grd@xc,...,\grd@xb}
        \node[anchor=north] at (\x,\grd@ya) {\pgfmathprintnumber{\x}};
        \foreach \y in {\grd@ya,\grd@yc,...,\grd@yb}
        \node[anchor=east] at (\grd@xa,\y) {\pgfmathprintnumber{\y}};
      }
    }
  },
  minor help lines/.style={
    help lines,
    step=\pgfkeysvalueof{/tikz/grid with coordinates/minor step}
  },
  major help lines/.style={
    help lines,
    line width=\pgfkeysvalueof{/tikz/grid with coordinates/major line width},
    step=\pgfkeysvalueof{/tikz/grid with coordinates/major step}
  },
  grid with coordinates/.cd,
  minor step/.initial=.2,
  major step/.initial=1,
  major line width/.initial=2pt,
}
\makeatother



==> media/traj-mc-ptp/insets/inset-mc-ptp.tex <==
% !TeX root = ../traj-mc-ptp.tex
% \clip (-9,-7) rectangle (9,7);
% \grid{-8}{-6}{4}{5}
\clip (-8,-6) rectangle (8,6);

% Ellipses
\DTLforeach*{mvar}{\letter=letter,\cx=cx,\cy=cy,\ang=ang,\sx=sx,\sy=sy,\nang=nang}{%
  \DTLifstringeq{\letter}{A}{\def\colpt{\colorA}}{}
  \DTLifstringeq{\letter}{B}{\def\colpt{\colorB}}{}
  \DTLifstringeq{\letter}{C}{\def\colpt{\colorC}}{}
  \DTLifstringeq{\letter}{Ap}{\def\colpt{\colorA}}{}
  \DTLifstringeq{\letter}{Bp}{\def\colpt{\colorB}}{}
  \DTLifstringeq{\letter}{Cp}{\def\colpt{\colorC}}{}
  \DTLifstringeq{\letter}{S}{\def\colpt{\colorS}}{}
  % \draw[draw=\colpt] (\cx,\cy) node[cross=0.5,\colpt]{};
  \coordinate (\letter) at (\cx,\cy);
  % \coordinate (C\letter) at ($(\cx,\cy)+(-60:\sx and \sy)$);
  \plotcovPTP{\cx}{\cy}{\ang}{\colpt}{\sx}{\sy}{\nang}{\letter}
}

\draw[black,thick] (-7.5,4.75) rectangle (3.5,-1);

% Points
\csvreader[head to column names,points]{ptp/ptsA.csv}{}{%
  \ifnum\idx=\numA
    \coordinate (scA) at (\cx,\cy);
  \fi
  \draw[fill=\colorA!25,draw=none] (\cx,\cy) circle [radius=0.05];
}
\csvreader[head to column names,points]{ptp/ptsB.csv}{}{%
  \ifnum\idx=\numB
    \coordinate (scB) at (\cx,\cy);
  \fi
  \draw[fill=\colorB!25,draw=none] (\cx,\cy) circle [radius=0.05];
}
\csvreader[head to column names,points]{ptp/ptsC.csv}{}{%
  \ifnum\idx=\numC
    \coordinate (scC) at (\cx,\cy);
  \fi
  \draw[fill=\colorC!25,draw=none] (\cx,\cy) circle [radius=0.05];
}
\csvreader[head to column names,points]{ptp/ptsAp.csv}{}{%
  \ifnum\idx=\numrA
    \coordinate (scAp) at (\cx,\cy);
  \fi
  \draw[fill=\colorA!15,draw=none] (\cx,\cy) circle [radius=0.05];
}
\csvreader[head to column names,points]{ptp/ptsBp.csv}{}{%
  \ifnum\idx=\numrB
    \coordinate (scBp) at (\cx,\cy);
  \fi
  \draw[fill=\colorB!15,draw=none] (\cx,\cy) circle [radius=0.05];
}
\csvreader[head to column names,points]{ptp/ptsCp.csv}{}{%
  \ifnum\idx=\numrC
    \coordinate (scCp) at (\cx,\cy);
  \fi
  \draw[fill=\colorC!15,draw=none] (\cx,\cy) circle [radius=0.05];
}
\csvreader[head to column names,points]{ptp/ptsS.csv}{}{%
  \ifnum\idx=\numS
    \coordinate (scS) at (\cx,\cy);
  \fi
  \draw[fill=\colorS!25,draw=none] (\cx,\cy) circle [radius=0.05];
}

% Sampled with prime
\draw[\colorA, thick, dashed] (scA) -- (scAp);
\draw[\colorB, thick, dashed] (scB) -- (scBp);
\draw[\colorC, thick, dashed] (scC) -- (scCp);
\draw[black, thick, dashed] (scS) -- (scAp);
\draw[black, thick, dashed] (scS) -- (scBp);
\draw[black, thick, dashed] (scS) -- (scCp);

% Sampled points
\draw[fill=\colorA,draw=none] (scA) circle [radius=0.07];
\draw[fill=\colorB,draw=none] (scB) circle [radius=0.07];
\draw[fill=\colorC,draw=none] (scC) circle [radius=0.07];
\draw[fill=\colorA,draw=none] (scAp) circle [radius=0.07];
\draw[fill=\colorB,draw=none] (scBp) circle [radius=0.07];
\draw[fill=\colorC,draw=none] (scCp) circle [radius=0.07];
\draw[fill=\colorS,draw=none] (scS) circle [radius=0.1];

% Centers
\pic[\colorA, very thick] at (A) {cross=0.2};
\pic[\colorB, very thick] at (B) {cross=0.2};
\pic[\colorC, very thick] at (C) {cross=0.2};
\pic[\colorA, very thick] at (Ap) {cross=0.2};
\pic[\colorB, very thick] at (Bp) {cross=0.2};
\pic[\colorC, very thick] at (Cp) {cross=0.2};
\pic[\colorS, very thick] at (S) {cross=0.2};

% Covariances descriptions
\draw[\colorS] (0,4.25) node{\Large $\bm{\Lambda}_j$};
\draw[\colorA] (-6,-1.5) node{\Large ${\widehat{\bm{\Sigma}}}^{1}_j$};
\draw[\colorB] (0,-1.5) node{\Large ${\widehat{\bm{\Sigma}}}^{2}_j$};
\draw[\colorC] (3,-1.5) node {\Large ${\widehat{\bm{\Sigma}}}^{3}_j$};

\pic[scale=0.8] at (-6.6,-0.2) {frame=$\mathcal{F}^L$/black/below left};


\draw[\colorA, latex-,very thick, shorten <=4pt] (Ap) to[bend left=25] (-6.5,4) node[above] {\Large $\bm{r}_1$};
\draw[\colorB, latex-,very thick, shorten <=4pt] (Bp) to[bend left=30] (-1.5,1.5) node[right] {\Large $\bm{r}_2$};
\draw[\colorC, latex-,very thick, shorten <=4pt] (Cp) to[bend right=30]  (2.75,-0.5) node[right]  {\Large $\bm{r}_3$};


==> media/traj-mc-ptp/insets/inset-traj.tex <==
% !TeX root = ../traj-mc-ptp.tex
%warthog and trajectory
% \grid{-3}{-6}{3}{5}
\clip (-3,-6) rectangle (3,6);

% Append points to series
\def\robotpath{}
\def\TApath{}
\def\TBpath{}
\def\TCpath{}
\def\TSpath{}
\csvreader[head to column names,trajectory]{trajectory/cov_traj.csv}{}{%
  \ifdefempty{\robotpath}{
      \eappto\robotpath{(\x,\y)};
      \eappto\TApath{(\xA,\yA)};
      \eappto\TBpath{(\xB,\yB)};
      \eappto\TCpath{(\xC,\yC)};
      \eappto\TSpath{(\xS,\yS)};
      \coordinate (aPath) at (\xA,\yA);
      \coordinate (bPath) at (\xB,\yB);
      \coordinate (cPath) at (\xC,\yC);
      \coordinate (sPath) at (\xS,\yS);
    }{
      \eappto\robotpath{ -- (\x,\y)};
      \eappto\TApath{ -- (\xA,\yA)};
      \eappto\TBpath{ -- (\xB,\yB)};
      \eappto\TCpath{ -- (\xC,\yC)};
      \eappto\TSpath{ -- (\xS,\yS)};
    }
}

%WARNING: override scope, ugly
\coordinate (R) at (-0.5,0);
\coordinate (theodolite) at (-1,3.5);

\begin{scope}
  %\draw[black, dashed, line width=1pt, -latex] \robotpath{};
  \draw[\colorA, line width=.5pt] \TApath{} node[right=0.1] {\large$\widehat{\mathcal{Q}}^1$};
  \draw[\colorB, line width=.5pt] \TBpath{} node[above=0.1] {\large$\widehat{\mathcal{Q}}^2$};
  \draw[\colorC, line width=.5pt] \TCpath{}  node[left=0.1] {\large$\widehat{\mathcal{Q}}^3$};
  \draw[\colorS, line width=.5pt] \TSpath{} node[above=0.1] {\large$\xi$};
  \csvreader[head to column names,trajectory]{trajectory/cov_traj.csv}{}{%
    \ifnum\idx=\idxTraj
      \coordinate (trajPA) at (\xA,\yA);
      \coordinate (trajPB) at (\xB,\yB);
      \coordinate (trajPC) at (\xC,\yC);
      \coordinate (trajPS) at (\xS,\yS);
    \fi
    \plotcovTraj{\xA}{\yA}{\angA}{\colorA}{\covxA}{\covyA}
    \plotcovTraj{\xB}{\yB}{\angB}{\colorB}{\covxB}{\covyB}
    \plotcovTraj{\xC}{\yC}{\angC}{\colorC}{\covxC}{\covyC}
    \plotcovTraj{\xS}{\yS}{\angS}{\colorS}{\covxS}{\covyS}
  }
  \pic[scale=\scaleRobot, rotate=\rotRobot] at (R) {warthog};
  \draw[\colorA, line width=.75pt, dash pattern=on 1pt off 1pt] \TApath{};
  \draw[\colorB, line width=.75pt, dash pattern=on 1pt off 1pt] \TBpath{};
  \draw[\colorC, line width=.75pt, dash pattern=on 1pt off 1pt] \TCpath{};
  \draw[\colorS, line width=.75pt, dash pattern=on 1pt off 1pt] \TSpath{};
  \pic[scale=\scaleRobot, rotate=\rotRobot] at (R) {warthogTop};
\end{scope}

%total stations frame
\pic[scale=1.2,rotate=-190] at (theodolite) {frame=$\mathcal{F}^W$/black/below left};



==> media/traj-mc-ptp/media-preamble.tex <==
\usetikzlibrary{positioning,calc,arrows.meta,math,shapes.misc,plotmarks}
\usepackage{amssymb,amsfonts,amsmath,amscd}
\usepackage{bm}

\usepackage{csvsimple}
\usepackage[utf8]{inputenc}
\usepackage{xstring}

% Trajectory variables
\def\rotRobot{55} %ugly but meh -> subpic do not rotate for weird reason
\def\scaleRobot{0.75}
\def\colorA{BrickRed}
\def\colorB{ForestGreen}
\def\colorC{RoyalBlue}
\def\colorS{Plum}
\def\idxTraj{0}

% PTP variables
\def\numS{60}
\def\numrA{46}
\def\numrB{77}
\def\numrC{9}
\def\numA{76}
\def\numB{35}
\def\numC{5}
% \def\allColors{\colorA,\colorB,\colorC}

% CSV import
\csvnames{trajectory}{
  idx=\idx,
  x=\x,y=\y,ang=\ang,covx=\covx,covy=\covy,
  xA=\xA,yA=\yA,angA=\angA,covxA=\covxA,covyA=\covyA,
  xB=\xB,yB=\yB,angB=\angB,covxB=\covxB,covyB=\covyB,
  xC=\xC,yC=\yC,angC=\angC,covxC=\covxC,covyC=\covyC,
  xS=\xS,yS=\yS,angS=\angS,covxS=\covxS,covyS=\covyS,
}
\csvnames{points}{
  idx=\idx,
  x=\cx,
  y=\cy,
}

% DAT
\usepackage{datatool}
% \DTLsetseparator{,}
\newcommand{\point}[2]{\DTLfetch{#1}{idx}{\num}{#2}}


% TIKZ
\tikzset{
   wheel/.pic={
        \draw[fill=black!40] (-1,-.7) rectangle ++ (2,1.4);
        \foreach \i in {-1,-.8,...,1}{ %change step here
            \draw (\i, -.7) -- (\i,.7);
        }
   },
   prism/.pic={
        \draw[fill=#1] circle(10pt);
        \draw[fill=black, rotate=45] (-10pt,0) -- (10pt,0);
        \draw[fill=black, rotate=-45] (-10pt,0) -- (10pt,0);
   },
   position/.pic={
        \draw[fill=#1] circle(5pt);
   },
   warthog/.pic={
   %wheels
        \pic[scale=.5*\scaleRobot, rotate=\rotRobot] at (-1.2,-1.0) {wheel};
        \pic[scale=.5*\scaleRobot, rotate=\rotRobot] at (1.2,-1.0) {wheel};
        \pic[scale=.5*\scaleRobot, rotate=\rotRobot] at (-1.2,1.0) {wheel};
        \pic[scale=.5*\scaleRobot, rotate=\rotRobot] at (1.2,1.0) {wheel};
    %robot
        % \fill[white, opacity=1] (-1.5,-1) rectangle ++(3,2);
        \draw[fill=Goldenrod] (-1.5,-1) rectangle ++(3,2);
    },
    warthogTop/.pic={
    %frame
        %\draw[stealth-stealth, thick] (.7,0) -- (0,0) node[below left, xshift=3pt, yshift=4pt]{$R$} -- (0,.7);
    %prisms
        \coordinate(p1) at (.6,-.8);
        \coordinate(p2) at (-1,.2);
        \coordinate(p3) at (1,.8);
        \coordinate(pRobot) at (0,-.3);
        \pic[scale=.7*\scaleRobot, rotate=\rotRobot] at (p1) {prism=\colorA};
        \pic[scale=.7*\scaleRobot, rotate=\rotRobot] at (p2) {prism=\colorB};
        \pic[scale=.7*\scaleRobot, rotate=\rotRobot] at (p3) {prism=\colorC};
        \pic[scale=.7*\scaleRobot, rotate=\rotRobot] at (pRobot) {position=\colorS};
    %dists
        % \draw[opacity=.7] (p1) -- ($(p1)!1.2!-90:(p2)$) edge[latex-latex, solid, opacity=1]node[midway, above, xshift=.2em, yshift=-.1em]{\small$\widehat{\alpha}$} ($(p2)!1.2!90:(p1)$) ;
        % \draw[opacity=.7] (p2) -- ($(p2)!1.2!90:(p1)$);

        % \draw[opacity=.7] (p1) -- ($(p1)!1.5!90:(p3)$) edge[latex-latex, solid, opacity=1]node[midway, right, xshift=-.1em]{\small$\widehat{\beta}$} ($(p3)!1.5!-90:(p1)$) ;
        % \draw[opacity=.7] (p3) -- ($(p3)!1.5!-90:(p1)$);

        % \draw[opacity=.7] (p2) -- ($(p2)!1.2!-90:(p3)$) edge[latex-latex, solid, opacity=1]node[midway, left, xshift=.2em, yshift=-.3em]{\small$\widehat{\gamma}$} ($(p3)!1.2!90:(p2)$) ;
        % \draw[opacity=.7] (p3) -- ($(p3)!1.2!90:(p2)$);
   },
   pics/frame/.style args={#1/#2/#3}{code={
        \draw[stealth-stealth, thick] (1,0) -- (0,0) -- (0,1);
        \fill (0,0) circle(2pt);
        \node[#3, color=#2] {\Large\textbf{#1}};
  }},
  pics/covarianceTraj/.style args={#1/#2/#3}{code={
        \draw[line width=.1pt, fill=#1] ellipse (#2 and #3);
        % \draw[thin,->,black] (-#2-.5,0) -- (#2+.5,0);
        % \draw[thin,->,black] (0,-#3-.5) -- (0,#3+.5);
  }},
  pics/covariancePTP/.style args={#1/#2/#3/#4/#5}{code={
        \draw[line width=.1pt, #1] ellipse (#2 and #3);
        \node(cov#5) at (#4:#2 and #3){};
        % \draw[thin,->,black] (-#2-.5,0) -- (#2+.5,0);
        % \draw[thin,->,black] (0,-#3-.5) -- (0,#3+.5);
  }},
  cross/.pic = {
  \draw (-#1,0) -- (#1,0);
  \draw (0,-#1) -- (0, #1);
  }
}

% Plot cov
\newcommand{\plotcovPTP}[8]{% x, y, angle, color, covx, covy, node angle, letter
  \pic[scale=.5,rotate=#3] at (#1,#2) {covariancePTP=#4/#5/#6/#7/#8};
  % \begin{scope}[yshift=1cm]
  % \end{scope}
}

\newcommand{\plotcovTraj}[6]{% x, y, angle, color, covx, covy
  \pic[scale=.5,rotate=#3] at (#1,#2) {covarianceTraj=#4/#5/#6};
  % \begin{scope}[yshift=1cm]
  % \end{scope}
}


% Grid
\newcommand{\grid}[4]{% x1, y1, x2, y2
  \draw(#1,#2) to[grid with coordinates] (#3,#4);
}
















